Exploiting On-chip Heterogeneity of Versal Architecture for GNN Inference Acceleration

Graph Neural Networks (GNNs) have revolutionized many Machine Learning (ML) applications, such as social network analysis, bioinformatics, etc. GNN inference can be accelerated by exploiting data sparsity in the input graph, vertex features, and intermediate data in GNN computations. For dynamic sparsity exploitation, we leverage the heterogeneous computing capabilities of AMD Versal ACAP architecture to accelerate GNN inference. We develop a custom hardware module that executes the sparse primitives of the computation kernel on the Programmable Logic (PL) and efficiently computes the dense primitives using the AI Engine (AIE). To exploit data sparsity during inference, we devise a runtime kernel mapping strategy that dynamically assigns computation tasks to the PL and AIE based on data sparsity. Our implementation on the VCK5000 ACAP platform leads to superior performance compared with the state-of-the-art implementations on CPU, GPU, ACAP, and other custom GNN accelerators. Compared with these implementations, we achieve significant average runtime speedup across various models and datasets of 162.42x, 17.01x, 9.90x, and 27.23x, respectively. Furthermore, for Graph Convolutional Network (GCN) inference, our approach leads to a speedup of 3.9-96.7x compared to designs using PL only on the same ACAP device.

==> 4_accelerator_design.tex <==
\section{Accelerator Design}

{\color{blue}{Figure of Hardware implementation of each kernel}}

%\subsection{Microarchitecture}


\subsection{AI Engine Array}

AI Engine is efficiently used to execute dense matrix multiplication. Update() Kernel is scheduled on the AIE array. AI Engine array Architecture can be divided into three operations: AI Engine tile, Data Movement, and  External Interface.

\subsubsection{AI Engine tile}
Each AIE tile contains the AI Engine and a memory module. The AI Engine is a highly-optimized processor featuring a single-instruction multiple-data (SIMD) and very-long instruction word (VLIW) processor that supports both fixed-point and floating-point precision. We take advantage of vectorization to improve the performance of matrix operations on ACAP AI engines. Using SIMD can greatly speed up computation by reducing the number of instructions required. At peak performance, each AIE is capable of performing 8 F32 MACs per cycle.  The weight matrix is loaded into the data memory of the AI Engine tile and distributed among the tiles.

{\color{blue}{Figure of F32 vectorization and memory distribution }}

For matrix sizes of MxN and NxL, a total of N F32 x F32 multiplications are required per output value. Therefore,
\[ number\,of\, computations\, required(NC) \equal M \times N \times L\]
Given that 8 32-bit MACs operations can be performed per cycle,
\[Compute\,bound \, for\,an\,AIE(CB)\equal NC/8\,cycles\,per\,AIE\]
To fully use the vector unit MAC performance, 8 32-bit multiplications are performed per cycle. From the vectorization figure, we understand that Vector w needs to store Nx32-bit in the vector register fetching data from the AI Engine data memory through the tile interface for each MAC operation for a column operation for a total of L times. Considering the data "h" needed for computation, it needs N x 32-bit data per cycle for a total of M times. But the AIE tile interface allows a maximum of two 256-bit loads per cycle. Given that we can perform a maximum of 8 MACs per cycle per AI Engine tile, 256-bit (8x32-bit)is enough for one vector MAC. Therefore, the memory bound (MB) of the AIE is greater of the two,
\[ MB\,for\,Matrix\,X\equal \frac{M\times N}{8} \]
\[ MB\,for\,Matrix\,Y\equal \frac{N\times L}{8} \]

A higher of the two, MB or CB, bound us to the number of cycles required by one AI Engine tile to execute the entire matrix multiplication H x W. 

To enhance our architecture, we employ numerous AIE tiles. However, we must work within certain restrictions that limit the number of AIE tiles we can use. One such limitation is the constrained data memory within each tile, which necessitates data movement to perform matrix multiplication fully. This creates a Memory Bound problem as only two 256-bit can be received, and only one 256-bit can be sent. Increasing the number of tiles will not necessarily improve performance. Additionally, we face a restriction on the number of external interfaces we can use to the PL, with a maximum of 39 array interface tiles available to the PL interface\cite{xilinxpl}.

To overcome these limitations, we have devised an efficient AIE array, as illustrated in the figure. We have grouped four AIE tiles into a computational core (CC), consisting of two rows with two AIE tiles in each row, with each tile connected to the adjacent one, resulting in data transfer only sideways. Each CC is responsible for executing a specific task with minimal data movement due to data dependencies within the task, thus efficiently utilizing the memory. Adding more tiles into a CC won't scale the performance in case of small matrix sizes. Making the matrix size of a task bigger also won't help due to limitations on memory. Every CC is connected to the FPGA fabric via one PL interface, enabling the execution of tasks of any size as each tile within the CC can work in a group of 1, 2, or 4, depending on the matrix size. For instance, for an 8x8 matrix, each tile can perform 1 row x 1 column without the need for accumulation with other rows and columns executed by the other tiles. In case the size is larger, intermediate MAC results are performed by other tiles and stored within the data memory, with data transferred to the next tile for accumulation. This arrangement of CCs improves the scalability and efficiency of our AIE array, allowing it to execute complex tasks effectively. There are 39 groups of these CC arranged to form the whole AI Engine array which is limited by the availability of array interface tiles. 
%Keeping these restrictions we work around building an effective AIE array. As shown in the figure, we group 4 AIE tiles together into a computational core (CC)(two rows with two AIE tiles in each row) such that each AIE tile is connected to the tile next to it. Therefore, the data transfer is only sideways. Each CC is responsible for executing a task (Section V C). Because of the data dependencies within the task the memory can be utilized efficiently with minimal data movement. Each CC has one PL interface where it is connected to the FPGA fabric. This arrangement of CC allows the execution of any size of the task as each tile within the CC can work in a group of 1,2,4 depending on the size of the matrix allotted. For example, if the size of a matrix is 8x8. Each tile can perform 1 row x 1 column. There won't be any need to accumulate with other rows and columns executed by the other tiles. If the size is bigger then intermediate MAC results are performed by other tiles and stored within the data memory and data is transferred to the next tile to accumulate.

% Each CC has a PL interface. So at once 39 tasks run in parallel. This arrangement makes use of the resources efficiently.


\subsubsection{Data Movement}

The cascade movement mechanism is utilized for efficient data transfer between the tiles in our architecture where the output of one tile is directly fed as the input to the next tile. Unlike regular interconnect, where a significant amount of data movement occurs between tiles leading to high latency and energy consumption, the cascade stream is processed in a pipeline, with each processing element directly passing its output to the next without any intermediate data storage or transfer. The data movement in our case is only sideways and this results in a greater advantage. The sideway connections enable us to exploit cascade movement effectively. For larger matrices, where data movement becomes a bottleneck, the cascade stream provides significant speedup over an interconnect-based approach with efficient resource utilization. Additionally, it minimizes data movement between tiles, resulting in reduced energy consumption and improved overall performance.



%We exploit the cascade movement mechanism for data transfer between the tiles. The output of one tile is then fed as the input to the next tile. As the data movement in our case is only sideways this gives a greater advantage over regular interconnect. Using an interconnect, there is a significant amount of data movement between tiles, which can result in high latency and energy consumption. On the other hand, with cascade stream, the data is processed in a pipeline, with each processing element passing its output directly to the next processing element, without the need for intermediate data storage or transfer. This can significantly reduce data movement and improve performance. So just having the sideway connections lets us exploit cascade movement. In larger matrices, where the data movement becomes a bottleneck, the cascade stream can provide significant speedup over an interconnect-based approach with efficient use of resources, and minimize the data movement between tiles, which can significantly reduce energy consumption and improve overall performance.

\subsubsection{External Interface}

As mentioned above the external interface to the FPGA fabric is through the PL interface (PLIO). PLIO provides high-bandwidth and low-latency connectivity between the PL and AI Engine array. We use the AXI4-Stream switch inside the AI Engine to connect to the AI Engine to PL interface (PLIO). This interface directly connects to the programmable Logic. PLIO has inbuilt asynchronous FIFOs to handle clock domain crossing.

We use AI Engine to NoC interface to connect the AXI4-Stream switch to the PS(ARM-Cortex-A72). The NoC interface also has a domain crossing between the clocks for AI Engine and the NoC. All the communications from the processor to AIE are made through the NoC.

Data transfer from DDR to the data memory of individual tiles is initiated by the ARM processor through the NoC. The DMA engine is configured for specific data transfer. This involves setting up the transfer direction, the source and destination addresses, and the transfer size. The data is transferred using the individual DMA engine of the AIE tile where it can directly access the DDR.
%AI Engine consists of 8 groups of 4 AI Engine tiles making it a total of 32 AI Engine tiles. Each group is responsible for executing a task (Section V C). The Weight matrix is loaded into the local memory of each tile from the DDR directly from the GMIO. BufferL at the upstream of the AIE array holds the feature matrix, which is transferred into the AIE through PLIO. Each AIE tile is connected to the tile next to it. The data transfer is only sideways. Each tile can perform 8 F32 data Multiply-Accumulates (MACs) per cycle.
 

\subsection{Arithmetic Logic Unit Array}

 Arithmetic Logic Unit(ALU) Array has $p_{sys}\times p_{sys}$ ALU units and three data buffers – BufferU, BufferO, and Result Buffer (RB). BufferO stores the graph adjacency matrix (A) and RB stores the output matrix. Each Buffer has $p_{sys}$ memory banks for parallel on-chip memory access. The graph Y is stored in the bank such that Y[i] is placed in $(i mod p_{sys})^{th}$ bank of BufferO. This makes O(N) to fetch a particular row or column of a matrix to 1 cycle. Each ALU is synthesized as a DSP and can execute various arithmetic operations, including multiplication, max, addition, etc. There is an interconnection network – Index Shuffle Network (ISN). ISN performs all-to-all interconnection between BufferU, BufferO, and the ALU array. ISN is required by the SpDMM and SpMM primitives for data routing. ISN takes the IR from BufferU and maps it with the right column or row from BufferO and sends it to the ALU array for processing. The Intermediate Result(IR) from the Update() on the AIE array is stored at BufferU is stored in row-major order using COO format. The task scheduler running on the ARM processor determines the sparsity of the graph and schedules the Aggregate() kernel on the ALU array as either SpDMM or SpMM primitive.

%The Intermediate Result(IR) from the Update() on the AIE array is stored at BufferU in sparse matrix format. The ALU array executes the Aggregate() kernel on either SpDMM or SpMM primitive. It has three data buffers – BufferU, BufferO, and Result Buffer (RB). BufferO stores the graph adjacency matrix (A) and RB stores the output matrix. Each Buffer has $p_{sys}$ memory banks (denoted bank 0 to bank $p_{sys} \minus 1$) for parallel on-chip memory access. Each ALU is synthesized as a DSP and can execute various arithmetic operations, including multiplication, max, addition, etc. 
%There is an interconnection network – Index Shuffle Network (ISN). ISN performs all-to-all interconnection between BufferU, BufferO, and the ALU array. ISN is required by the SpDMM and SpMM primitives for data routing.
%ISN takes the IR from BufferU and maps it with the right column or row from BufferO and sends it to the ALU array for processing. 
%The required data format and layout for various execution modes are summarized in Table.

%\textbf{GEMM Mode:} The ALU array is organized as a two-dimensional systolic array to execute GEMM using output stationary dataflow [13]. The two input matrices are stored in BufferO and BufferP using the dense format. The systolic array can execute $p^2_{sys}$ multiply-accumulate (MAC) operations per clock cycle.



In SpDMM primitive, the ALU array is divided into two halves. The first half multiplies and passes to the second half where the products are accumulated. The dense matrix is stored in BufferO. Each non-zero element from the BufferU is fetched by the ISN and it selects a value from BufferO that matches the row-column and form a pair which is routed to the ALU array where it is first multiplied and passed on to the next phase where its accumulated ad stored in the result buffer.

In the case of the SpMM primitive, both Buffer[U/O] contain sparse matrices. We use only two columns of the ALU array forming $p_{sys}$ parallel computation pipelines. ISN fetches a non-zero value from BufferU and its pair from BufferO and forms a pair. The first column multiplies the pair and the second column adds it up. 
Each pipeline also has a Sparse Data Queue (SQ) to store the intermediate results in a sparse format.

Running the SpMM and SpDMM primitives on the ALU array efficiently skips the computation of non-zero elements in a sparse matrix improving the execution time and saving energy.
%\textbf{SpDMM Mode:} The ALU array is divided into $p_{sys}/2$ Update Units and $p_{sys}/2$ Reduce Units. Each Update or Reduce Unit has an ALU array of size $p_{sys}/2\times2$. Multiplication of a sparse matrix with a dense matrix is executed using the ScatterGather Paradigm shown in Algorithm 2. The sparse matrix denoted as X (in BufferU) is stored in row-major order using COO format. The dense matrix denoted as Y (in BufferO) is stored in row-major order using the dense format, and Y [i] is stored in the bank (i mod $p_{sys}$) of BufferO. Each non-zero element e(i, j, weight) in X is fetched from the BufferU ($p_{sys}/2$ elements can be fetched from BufferU per cycle) and sent to the ISN. Then e is routed to the bank (i mod $p_{sys}$) for fetching Y [i], which forms the input data pair (Y [i], e). The input pair is routed to the (j mod $p_{sys}/2)^{th}$ Update Unit. The Update Unit performs the multiplication of e.value and Y [i] to produce the intermediate result u. Then the corresponding Reduce Unit adds u to Z[j]. SpDMM Mode can efficiently skip zero elements in the sparse matrix X. The SpDMM Mode can execute $p^2_{sys}/2$ multiply-accumulate (MAC) operations per clock cycle (The $p^2_{sys}/2$ Update Units can execute $p^2_{sys}/2$ multiply operations and the $p^2_{sys}/2$  Reduce Units can execute $p^2_{sys}/2$ addition operations).

%\textbf{SpDMM Mode:} The ALU array is divided into $p_{sys}/2$ Update Units and $p_{sys}/2$ Reduce Units. Each Update or Reduce Unit has an ALU array of size $p_{sys}/2\times2$. Multiplication of a sparse matrix with a dense matrix is executed using the ScatterGather Paradigm shown in Algorithm 2. The sparse matrix denoted as X (in BufferU) is stored in row-major order using COO format. The dense matrix denoted as Y (in BufferO) is stored in row-major order using the dense format, and Y [i] is stored in the bank (i mod $p_{sys}$) of BufferO. Each non-zero element e(i, j, weight) in X is fetched from the BufferU ($p_{sys}/2$ elements can be fetched from BufferU per cycle) and sent to the ISN. Then e is routed to the bank (i mod $p_{sys}$) for fetching Y [i], which forms the input data pair (Y [i], e). The input pair is routed to the (j mod $p_{sys}/2)^{th}$ Update Unit. The Update Unit performs the multiplication of e.value and Y [i] to produce the intermediate result u. Then the corresponding Reduce Unit adds u to Z[j]. SpDMM Mode can efficiently skip zero elements in the sparse matrix X. The SpDMM Mode can execute $p^2_{sys}/2$ multiply-accumulate (MAC) operations per clock cycle (The $p^2_{sys}/2$ Update Units can execute $p^2_{sys}/2$ multiply operations and the $p^2_{sys}/2$  Reduce Units can execute $p^2_{sys}/2$ addition operations).

%\textbf{SpMM Mode:} The ALU array is organized as $p_{sys}$ parallel Sparse Computation Pipelines (SCP) as shown in Figure. Each SCP has two ALUs to perform the multiplication of two non-zero elements and the merging of intermediate results. Each SCP also has a Sparse Data Queue (SQ) to store the intermediate results in a sparse format. The multiplication of two input sparse matrices is executed using the Row-wise Product with Scatter-Gather paradigm as shown in Algorithm 3. For Row-wise Product, a row Z[j] of output matrix Z is calculated through: 
%\[Z[j] = \Sigma_i X[j][i] \ast Y [i]\]      (3) 
%For calculating the output matrix Z, an SCP is assigned the workload of a row of the output matrix (Equation 3). $p_{sys}$ SCPs can calculate $p_{sys}$ output rows in parallel until all the rows of the output matrices are calculated. To efficiently execute Row wise Product, all input sparse matrices (X, Y ) and output matrices are stored using COO format in row-major order. Using SpMM Mode, we can skip the zero elements in both the input matrices. SpMM Mode can execute $p_{sys}$ multiply-accumulate (MAC) operations per clock cycle. \\
%\textbf{Mode switching:} The execution mode is set by the control bits of the hardware multiplexers in ACM. The overhead of switching execution modes is just one clock cycle. \\
%\textbf{Trade-off:} The three execution modes have different ways of dealing with non-zero elements in the two input matrices. Therefore, their execution time of multiplying two input matrices depends on the data sparsity. We analyze the trade-off of the three execution modes w.r.t. data sparsity in Section.





\section{Algorithm}

\subsection{Partitioning algorithm}
Using the GCN model defined in the Pytorch Geometric Library and the metadata as input, the compiler can generate the GNN matrices. The first step of the proposed algorithm is partitioning the graphs into sub-graphs. 

The adjacency matrix $\bm{A}$ with dimension ${|\mathcal{V}|} \times {|\mathcal{V}|}$ will be partitioned into blocks with size ${N}_1$ $\times$ ${N}_1$. 
%$\bm{Aij}$ will represent the block that $\bm{Aij}$ = $\bm{A}$ [i * ${N}_1$ : (i+1) * ${N}_1$][j * ${N}_1$ : (j+1) * ${N}_1$]. 
The feature matrix $\bm{H}$ with dimension ${|\mathcal{V}|} \times {{f}_1}$ will be partitioned into fiber ${N}_1$ $\times$ ${N}_2$. 
%Each fiber $\bm{H}_ij$ = $\bm{A}$ [i * ${N}_1$ : (i+1) * ${N}_2$][j * ${N}_1$ : (j+1) * ${N}_2$]. 
Each fiber is further broken down into size ${N}_2$ $\times$ ${N}_2$ to match the block size of weight matrix $\bm{W}$. We denote ${H}_{ij-k}$ as the ${k}^{th}$ sub-fiber of $\bm{H}_ij$. The weight matrix $\bm{W}$ has dimension ${f}_1 \times {f}_2$. It is partitioned into blocks with size ${N}_2$ $\times$ ${N}_2$.
%where $\bm{W}_ij$ = $\bm{W}$ [i * ${N}_2$ : (i+1) * ${N}_2$][j * ${N}_2$ : (j+1) * ${N}_2$].

 %\textbf{Prepossessing Partitions}: when partitioning the graph, the compiler will obtain the sparsity of each partition. The hardware will acquire the sparsity of intermediate results at run-time. 
\subsection{Dynamic Mapping}

The execution of a kernel contains independent computation tasks that each compute an output data partition. We implement dynamic scheduling on the PL region when executing the Aggregate() kernel. Depending on the sparsity of the input matrices, the ARM processor will map each computation task to SpMM or SpDMM and skip any empty input matrix. The proposed mapping can ensure the best parallelization by exploiting data sparsity for the Aggregate() kernels. As each task is independent, mapping the next task can happen before finishing the current task. 

\subsection{Task scheduling}
We proposed an intralayer pipelining strategy to optimize the heterogeneous system. The scheduler maps the Update() kernel onto the AIEs as it contains mainly GEMM. In contrast, the Aggregate() kernel will be dynamically mapped onto PL based on the sparsity of the partition, as mentioned in the subsection above. 
In a two layers GCN inference, there will be intermediate results within each layer after the first-layer Update() and second-layer Update() ($\bm{G1}$, $\bm{G2}$). When running the first-layer Update() tasks executing $\bm{H} \times \bm{W}$, the scheduler will run tasks that produce the results of the partition $\bm{G1}_{ij}$ with the shape of $\bm{N}_{1} \times \bm{N}_{2}$. 
%$\bm{G1}_{ij}$ = $\bm{G1}$ [i * ${N}_1$ : (i+1) * ${N}_2$][j * ${N}_1$ : (j+1) * ${N}_2$]. 
Once partition $\bm{G1}_{00}$ is computed, the scheduler will start scheduling the Aggregate() tasks. We move on to the second layer only when all the computations of one layer are executed (Algorithm \ref{alg: Tasks}).

%At the start of runtime, AIE will begin working on the Update() kernel, while the PL region will remain IDLE before $\bm{G1}_{ij}$ is computed. Once $\bm{G1}_{ij}$ is passed over through PLIO to the PL On-chip memory, the compiler will start scheduling tasks from the Aggregate() Kernel on the PL (Algorithm \ref{alg: Task Scheduling}). With the pipelining strategy, the Aggregate() or Update() tasks can be hidden depending on the latency. The same thing applies to $\bm{G2}$. We move on to the second layer only when all the computations of one layer are executed. 

\begin{algorithm}
\caption{Task Scheduling for the Whole System}
\label{alg: Tasks}
\begin{small}
\begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
 \Require Input: Partitions of A, H, W, The numbers of Layers L
 \Ensure Output: Output of GCN model;
\For{$l$ = 1 to L} //schedules two kernels in parallel
    \For {Task in Update() Kernel $l$ \textbf{parallel}} 
    \If{There is an idle AIE CC:} 
    \State{Assign this task to CCi on AIE}
    \EndIf 
    \EndFor
    \For {Task in Aggregate() Kernel $l$ \textbf{parallel}}
    \If{There is an idle PL CC and ${G}_{ij}$ is received:} 
    \State{Assign this task to CCi on PL}
    \EndIf 
    \EndFor
\State{Move to next layer once all the Kernels are done}

\EndFor
\end{algorithmic}
\end{small}
\end{algorithm}

%\begin{algorithm}
%\caption{Pipelined Task Scheduling on PL }
%\label{alg: Task Scheduling}
%\begin{small}
%\begin{algorithmic}[1]
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}
% \Require Input: Partitions of A and ${G1}_{ij}$
% %$\left\{\bm{H}_{0,0}, ..., %\bm{H}_{\frac{|\mathcal{V}|}\mathcal{N}_{2}},\frac{f_{1}}%%{\mathcal{N}_{2}}}\right\}$, $\left\\bm{W}_{0,0}, ..., %\bm{H}_{\frac{f_{1}}%\mathcal{N}_{2}},\frac{\mathcal{f}_{2}}%{\mathcal{N}_{2}}}\right\}$;
% \Ensure Output: Intermediate Results of GCN model;
%\For{i in $\frac{f_{1}}{\mathcal{N}_{2}}$}
%\For{j in $\frac{|\mathcal{V}|}{\mathcal{N}_{1}}$}
%\State{Waiting for ${G1}_{ij}$ from AIE:}
%        \State{$\rightarrow$Start scheduling Aggregate() tasks with ${G1}_{ij}$}
%\EndFor
%\EndFor
%\end{algorithmic}
%\end{small}
%\end{algorithm}

\subsection{Performance Model}

The performance model calculates the computation time of each primitive. The computation time of SpDMM and SpMM on the PL depends on the data sparsity of the matrices X and Y. The density of X and Y are $\alpha_X$ and $\alpha_Y$ respectively, while $X\in\mathbb{R}^{mxn}$ and $Y\in\mathbb{R}^{nxd}$.
\begin{center}
\begin{tabular}{c c c c}
 \hline
  & Update() &  \multicolumn{2}{c}{Aggregate()} \\ 
 \hline
 Process & GEMM & SpDMM & SpMM \\ [0.5ex] 
 \hline
 MACs per Cycle & {8*\#AIE} & $p^2_{sys}$ / 2& $p_{sys}$ \\ 
 \hline
 Execution time & $\frac{mnd}{8*\#AIE}$ & $\alpha_{min}\frac{2mnd}{p^2_{sys}}$ & $\alpha_X\alpha_Y\frac{2mnd}{p_{sys}}$\\
 \hline
 Frequency & $\textit{f}_{AIE}$ & $\textit{f}_{PL}$ & $\textit{f}_{PL}$ \\
\end{tabular}
\end{center}

For Update() tasks, two input matrices are considered dense matrices, and the GEMM unit can process {8*\#AIE} MACs per cycle as the one AIE tile can compute eight FP32 MACs in a cycle. More parallelism can be achieved by increasing the tiles used for the matrix multiplication process. To calculate the more accurate run time of the AIE, the MACs per cycle will need to multiply by the efficiency of each AIE tile. 

%The Aggregate() tasks will be mapped onto SpMM and SpDMM. In SpMM mode, the computation core skips all the zeros in both matrices and performs $p_{sys}$ MACs per cycle. In SpDMM mode, the computation ignores the zeros in one of the input matrices and performs $p^2_{sys}$ MACs per cycle.  

%For executing Aggregate(), when $\alpha_{max} \geq \frac{2}{p_{sys}}$ , SpDMM mode will be the best. When $\alpha_{max} < \frac{2}{p_{sys}}$, SpMM mode will have the least execution time. We denote $\alpha_{max} $= Max($\alpha_X\alpha_Y$). In the Aggregate() process, we observed that there is only $<$ no of dense matrix multiplication in total aggregate() tasks. Thus, mapping those onto SpDMM will not affect the latency. 


\section{Implementation Details}
%1/4 page\\
%{\color{blue}{Which platform we are using}}
We implement the proposed accelerator on a state-of-the-art VCK5000 ACAP board. For CC, $p_{sys} \equal 16$. We develop the CC using Verilog HDL and implement the soft processor using ARM cortex-A72 part of Control, Interfaces and Processing System (CIPS) IP \cite{xilinxcips}. AIE Array and CC are connected to the soft processor through the PLIO and AXI4-Stream interface, respectively, through which the soft processor sends the control signals to the AIE array, and the CC sends the sparsity information to the soft processor. We develop the Compiler using Python on the Host Processor (Intel Xeon 5120 CPU) and develop the Runtime system on the soft processor using C++ in Xilinx Vitis Unified Software Platform (version 2021.2). The Index Shuffle Network and Data Shuffle Network are implemented using a butterfly network with buffering to handle the routing congestion. We perform synthesis and Place \& Route using Vivado 2021.2. The resource utilization is summarized in the table. The CCs run at 297 MHz.
